Continuous One-Counter Automata

We study the reachability problem for continuous one-counter automata, COCA for short. In such automata, transitions are guarded by upper and lower bound tests against the counter value. Additionally, the counter updates associated with taking transitions can be (non-deterministically) scaled down by a nonzero factor between zero and one. Our three main results are as follows: (1) We prove that the reachability problem for COCA with global upper and lower bound tests is in NC2; (2) that, in general, the problem is decidable in polynomial time; and (3) that it is decidable in the polynomial hierarchy for COCA with parametric counter updates and bound tests.

==> flat-parametric.tex <==
\subsection{Basic properties}

In this subsection, we establish basic properties of paths and cycles
of a guarded COCA $\W = (Q, T, \tau)$.

\begin{lemma}\label{lemma:follower}
  Let $t \in T$, $\alpha, \beta \in (0, 1]$ and $a, a', b, b' \in \Q$
    be such that $a' = a + \alpha \Effect{t}$ and $b' = b + \beta
    \Effect{t}$. If $a \leq b$ and $a' \geq b'$, then $b' = a +
    \alpha' \Effect{t}$ and $a' = b + \beta' \Effect{t}$ for some
    $\alpha', \beta' \in (0, 1]$.
\end{lemma}

\begin{proof}
  The claim is trivial whenever $a = b$ or $a' = b'$, hence assume $a
  < b$ and $a' > b'$. Note that $\Effect{t} \neq 0$, as we would
  otherwise derive the contradiction $a < b = b' < a' = a$. Let
  \[
    \alpha' \defeq \dfrac{b' - a}{\Effect{t}} \text{ and }
    %
    \beta' \defeq \dfrac{a' - b}{\Effect{t}}.
  \]
  We have $a + \alpha' \Effect{t} = b'$ and $b + \beta' \Effect{t} =
  a'$ as desired. It remains to show that $\alpha', \beta' \in (0,
  1]$. From $a' > b'$, we have:
  \begin{alignat*}{4}
    \alpha'
    &=\ & (b' - a) / \Effect{t}
    &<\ & (a' - a) / \Effect{t}
    &=\ & \alpha \leq 1, \\
    %
    \beta'
    &=\ & (a' - b) / \Effect{t}
    &>\ & (b' - b) / \Effect{t}
    &=\ & \beta > 0.
  \end{alignat*}
  From $a < b$, we symmetrically derive $\alpha' > 0$ and $\beta' \leq
  1$.
\end{proof}

\begin{lemma}\label{lem:convex}\label{lemma:convex}
  Let $\pi$ be a path, let $a, a', b, b' \in \Q$ and let $\Lambda \in
    (0, 1]$. If $a \steps{\pi} a'$ and $b \steps{\pi} b'$, then $(1 -
    \Lambda) a + \Lambda b \steps{\pi} (1 - \Lambda) a' + \Lambda b'$.
\end{lemma}

\begin{proof}
  We prove the case where $\pi$ is a transition $t$. The general case
  follows by induction. By definition, there exist $\alpha, \beta \in
    (0, 1]$ such that $a \steps{\alpha t} a'$ and $b \steps{\beta t}
    b'$. Let $\gamma \defeq (1 - \Lambda) \alpha + \Lambda
    \gamma$. Clearly, $\gamma \in (0, 1]$ by convexity and since $(0,
    1]$ is an interval. Hence, we are done since:
  \begin{alignat*}{2}
        & [(1 - \Lambda) a + \Lambda b] + \gamma \Effect{t}                           \\
    %
    =\  & [(1 - \Lambda) a + \Lambda b] + [(1 - \Lambda) \alpha +
    \Lambda \beta] \Effect{t}                                                         \\
    %
    =\  & (1 - \Lambda)(a + \alpha \Effect{t}) + \Lambda (b + \beta
    \Effect{t})                                                                       \\
    %
    =\  & (1 - \Lambda) a' + \Lambda b'.                            & \tag*{\qedhere}
  \end{alignat*}
\end{proof}

\begin{proposition}\label{prop:path:interval}
  For every path $\pi$ and every cycle $\Theta$, the sets
  $\Post{\pi}{x}$ and $\Post{\Theta^+}{x}$ are intervals.
\end{proposition}

\begin{proof}
  We first prove the property for $\pi$.
  Assume $|\Post{\pi}{x}| > 1$, as we are otherwise done. Let $a, c
    \in \Post{\pi}{x}$ be such that $a < c$. We show that any $b \in
    (a, c$) belongs to $\Post{\pi}{x}$. We have $x
  \steps{\pi} a$ and $x \steps{\pi} c$.
  Moreover, $b = (1 - \Lambda) a + \Lambda c$ for some $\Lambda
  \in (0, 1)$. By \autoref{lem:convex}, 
  we have $x \steps{\pi} b$ and hence $b \in
  \Post{\pi}{x}$. So the claim holds for $\pi$.

  Next, we prove the claim for $\Theta$.
  Let us assume that $|\Post{\theta^+}{x}| > 1$, as we are otherwise
  done. Let $a, c \in \Post{\theta^+}{x}$ be such that $a <
  c$. We must show that any $b \in (a, c)$ belongs to
  $\Post{\theta^+}{x}$. By definition, there exist 
  runs $\sigma, \rho$ such that $x \steps{\sigma} a$,
  $x \steps{\rho} c$ and $\upath{\sigma}, \upath{\rho} \in \theta^+$. Let
  $\Theta = t_1 \dots t_n$, $\sigma = \alpha_1 t_1 \dots \alpha_m t_m$, $\rho = \gamma_1 t_1 \dots \gamma_m' t_m'$.

  Note that if $\effect{t} = 0$ for all $t \in \theta$, clearly
  $\Post{\Theta^+}{x} \subseteq \{x\}$, so the claim holds.
  Then suppose that $\effect{t} < 0$ for some $t \in \pi$. 
  The positive case is symmetric.

  Let us construct a run $\phi$ such that $\upath{\phi} \in \theta^+$ and $\Effect{\phi} =
  b - x$.

  Let us first argue the case $b = x$.
  Then let us define for $1 \leq i \leq n$
  \begin{gather*}
    \beta_i = \begin{cases} 1/\rho_{+} & \text{if } \effect{t_i} \geq 0 \\
      -1/\rho_{-} & \text{if } \effect{t_i} < 0
    \end{cases},
  \end{gather*}
  where $\Theta_+ = \sum_{i \leq n} max(0, \effect{t_i})$ and $\Theta_- = \sum_{i \leq n} min(0, \effect{t_i})$.
  Note that because $a < b = x < c$, there must be some $t, t' \in \Theta$ such that
  $\effect{t} > 0$ and $\effect{t} < 0$.
  Additionally, we can assume effects of transitions to be integers.
  Hence $\rho_{-} \leq -1$ and $\rho_{+} \geq 1$.
  Then we define $\phi = \beta_1 t_1 \dots \beta_n t_n$. It holds that
  $x + \effect{\phi} =  x + 1/\rho_{+} \rho_{+} - 1/\rho_{-} \rho_{-} = x$.
  So $\phi$ has the right effect, and it only remains to argue about its admissibility from $x$.
  
  Now, let us argue the case $b > x$; the case $b < x$ is symmetric.
  In this case, it holds that $c > b > x$.
  Then let us define $\phi = (b-x)/(c-x) \rho$.
  It holds that $\phi$ is a run, since $(b-x)/(c-x) \in \ZeroOne$.
  Further, it holds that $x + \effect{\phi} = x + (b-x)/(c-x) (c-x) = x + b - x = b$.

  

  Let us construct a
  run $\phi$ such that $\upath{\phi} \in \theta^+$ and $\Effect{\phi} =
  b - x$. If $b \geq x$, then we can take $\phi \defeq \beta \rho$ for a
  suitable $\beta \in (0, 1]$ since $\Effect{\rho} = c - x > b -
  x$. If $b < x$, then we first rescale $\rho$ into a run $\rho'$
  with negative effect. Formally, let $\rho' \defeq \alpha_1' t_1
  \cdots \alpha_n' t_n$ where
  \[
  \alpha_i' \defeq
  \begin{cases}
    1 / (2n \cdot \Effect{t_i})
    & \text{if $\Effect{t_i} > 0$}, \\
    %
    1
    & \text{otherwise}.
  \end{cases}
  \]
  We have $\Effect{\rho'} \leq 1/2 - 1 = -1/2$ and hence
  $\Effect{\beta \rho'} = -1/2$ for some $\beta \in (0, 1]$. Let $\phi
  \defeq (\beta \rho')^{2(c - b')}$. We have $\effect{\phi} = b' -
  c$. So again, $\phi$ has the right effect, and it remains
  to show admissibility from $x$.

  If run $\phi$ is admissible from $c$, then we are done as we obtain
  $x \steps{\phi} b$. Otherwise, let $a_i \defeq x +
  \Effect{\FromTo{\sigma}{1}{i}}$, $b_i \defeq x +
  \Effect{\FromTo{\phi}{1}{i}}$ and $c_i \defeq x +
  \Effect{\FromTo{\rho}{1}{i}}$. There exists a maximal $j < |\phi|$
  such that one of these two cases holds: $b_j \not\in
  \botguard{\Out{\phi_j}}$ or $b_j \not\in \topguard{\Out{\phi_j}}$.

  \begin{figure}
    \begin{center}
      \input{fig-interval-merge}
    \end{center}
    \caption{\emph{Gray blocks}: guards; \emph{solid black}: runs $x
      \steps{\sigma} a$ and $x \steps{\rho} c$; \emph{dashed red}:
      inadmissible run $\phi$ from $x$ to $b$; \emph{filled blue}:
      combined run $x \steps{\pi^+} b$.}%
    \label{fig:interval:merge}
  \end{figure}

  \emph{Case 1:} Although $\phi$ and $\sigma$ may not have the same
  length, they both use $\pi$. So, each nonfinal state of $\phi$ has
  (at least) one counterpart in $\sigma$ with the same outgoing
  transition. Formally, for each $i < |\phi|$, there is some $f(i) <
  |\sigma|$ with $\phi_{i+1} = \sigma_{f(i)+1}$. Since $\sigma$ is
  admissible from $x$, there is a maximal $\ell$ such that $j \leq
  \ell < |\phi|$ and $b_\ell < a_{f(\ell)}$. In particular,
  $b_{\ell+1} \geq a_{f(\ell)+1}$. Thus, we may combine the two runs
  with \autoref{lemma:follower} (see~\autoref{fig:interval:merge}):
  \[
  x \steps{\FromTo{\sigma}{1}{f(\ell)}} a_{f(\ell)}
  \steps{\sigma_{f(\ell) + 1}} b_{\ell+1}
  \steps{\FromTo{\phi}{\ell+2}{|\phi|}} b.
  \]
  \emph{Case 2:} It is symmetric. More precisely, we define $f$
  w.r.t.\ $\rho$, take $\ell \geq j$ such that $b_\ell > c_{f(\ell)}$
  and $b_{\ell+1} \leq c_{f(\ell)+1}$, and obtain:
  \[
  x \steps{\FromTo{\rho}{1}{f(\ell)}} c_{f(\ell)} \steps{\rho_{f(\ell) +
      1}} b_{\ell+1} \steps{\FromTo{\phi}{\ell+2}{|\phi|}}
  b. \qedhere
  \]
\end{proof}

\begin{proposition}\label{prop:thetatwo}
  For every cycle $\Theta$, it is the case that $\enab{\Theta^2}$
  equals $\emptyset$ or $\enab{\Theta}$, and $\enab{\Theta^2} =
  \enab{\Theta^3} = \cdots$.
\end{proposition}

\begin{proof}
  Note that by definition, it holds that $\cdots \subseteq \enab{\Theta^3} \subseteq \enab{\Theta^2} \subseteq \enab{\Theta}$.
\end{proof}

\subsection{Symbolic representation of reachability functions}

\newcommand{\PPost}[2]{\ifempty{#2} \mathrm{Post}_{#1}^\mu \else \mathrm{Post}_{#1}^\mu(#2) \fi}
\newcommand{\Penab}[1]{\mathrm{enab}^\mu(#1)}
\newcommand{\less}[1]{#1_{-}}
\newcommand{\more}[1]{#1_{+}}

Let us fix a parametric COCA $\Pp = (Q, T, \tau, Y)$. Let
$\PPost{\pi}{x}$ and $\Penab{\pi}$ denote the function $\Post{\pi}{x}$
and set $\enab{\pi}$ of the guarded COCA $\Pp^\mu$. Now that we
know that $\PPost{\pi}{x}$ and $\PPost{\Theta^+}{x}$ are intervals, we
seek to provide an effective \emph{symbolic} representation of these
intervals that handles $x$ and valuation $\mu$ in a \emph{uniform}
way.

As such intervals can be open or closed on the left or right depending
on $x$ and $\mu$, it will be convenient to extend $\Q$ with ``limit''
elements. Let $\less{\Q} \defeq \{\less{a} : a \in \Q\}$ and
$\more{\Q} \defeq \{\more{a} : q \in \Q\}$ be disjoint copies of
$\Q$. Informally, $\less{a}$ and $\more{a}$ stand for $a - \delta$ and
$a + \delta$ where $\delta$ is infinitesimal. We extend addition and
comparison as follows using symbols $\oplus$ and $\prec$ to avoid
confusion. For every $a, b \in \Q$, let $a \oplus b \defeq a + b$ and
$a \prec b \iff a < b$ in the standard way, and let
\begin{align*}
  \less{a} \oplus b &= b \oplus \less{a} = \less{a} \oplus \less{b} =
  \less{(a \oplus b)}, \\  
  %
  \more{a} \oplus b &= b \oplus \more{a} = \more{a} \oplus \more{b} =
  \more{(a \oplus b)}, \\  
  %
  \less{a} \prec b & \text{ if $a \leq b$ and $\less{a} > b$ otherwise}, \\
  %
  \more{a} \succ b & \text{ if $a \geq b$ and $\more{a} < b$ otherwise}.
\end{align*}
\philip{do we also need to extend multiplication? it seems we need it for linear combinations}
Elements $-\infty$ and $+\infty$ further behave as expected,
e.g.\ $-\infty \prec \less{3} \prec \more{3} \prec +\infty$ and
$\less{3} \oplus +\infty = +\infty$. Note that $\prec$ is a total
order. Moreover, the addition of elements of $\more{\Q}$ and
$\less{\Q}$ is undefined as we never need to carry such
operations. This stems from the fact that these two sets are only
useful to specify openness on the right and left, respectively. For
example, with this notation the interval $I \defeq (3, 5]$ can be
  written as $[\more{3}, 5]$ which stands for $\{a \in \Q : \more{3}
  \preceq a \preceq 5\}$. Hence, in this example, we have $\inf I =
  \more{3}$ and $\sup I = 5$.

Let us now introduce our data structure for $\PPost{\pi}{x}$. We
assume that the parameters $Y = \{y_1, \ldots, y_k\}$ of $\Pp$ are
partitioned into two sets $Y^{-}$ and $Y^{+}$. This allows us to
distinguish parameters that hold negative and positive values. This
partition will later be guessed by a nondeterministic Turing machine
towards the end of this section. Consequently, we say that a parameter
valuation $\mu$ is \emph{consistent} if $y \in Y^{-}$ iff $\mu(y) < 0$
and $y \in Y^{+}$ iff $\mu(y) > 0$. In particular, this means that we
will not consider zero valuations.

A \emph{linear expression} is a term of the form $a_1 y_1 \oplus
\ldots \oplus a_k y_k \oplus b$ where $a_1, \ldots a_k \in \Q_{\geq
  0}$ and $b \in \Q \cup \less{\Q} \cup \more{\Q} \cup \{-\infty,
+\infty\}$. We say that such a term is a \emph{left} expression if $b
\in \Q \cup \more{\Q} \cup \{-\infty\}$, or a \emph{right} expression if
$b \in \Q \cup \less{\Q} \cup \{+\infty\}$. Furthermore, a left expression
is \emph{negative} if $b \in \cup_{c \in \Q_{\leq 0}} \{c, \more{c}\}$
and $a_i \neq 0$ implies $y_i \in Y^{-}$, and a right expression is
\emph{positive} if $b \in \cup_{c \in \Q_{\geq 0}} \{c, \less{c}\}$
and $a_i \neq 0$ implies $y_i \in Y^{+}$. For example, if $Y^{-} =
\{y_1, y_2\}$ and $Y^{+} = \{y_3, y_4\}$, then $y_1 \oplus 3 y_2
\oplus (-7)$ and $y_4 \oplus \less{0}$ are respectively negative and
positive. We will write $\varphi^\mu$ to denote the value obtained by
substituting parameters occurring in the linear expression $\varphi$
by their value under valuation $\mu \colon Y \to \Q$.

Let $\mathcal{F} = \{f^\mu \colon \Q \to \intervals\}_{\mu \in V}$ be
a family of functions where $V$ is a set of consistent valuations, and
$f^\mu$ is a function associated to $\mu \in V$. We say that
$\mathcal{F}$ is a \emph{threshold interval} if there exist a negative
linear expression $\Psi_{\max}$, a positive linear expression
$\Psi_{\min}$, and finite collections $E_{\max}$ and $E_{\min}$ of
left and right linear expressions such that:
\begin{align*}
  f^\mu(x)
  %
  &=
  [\max(x \oplus \Psi_{\max}^\mu, \max_{\varphi \in E_{\max}}
    \varphi^\mu),\
  %
  \min(x \oplus \Psi_{\min}^\mu, \max_{\varphi \in E_{\min}}
    \varphi^\mu)].
\end{align*}
The \emph{size} of such a threshold interval is $|E_{\max}| +
|E_{\min}|$. We say that a threshold interval is \emph{effective} if
its representation can be computed in polynomial time w.r.t.\ the
description of $\mathcal{F}$.

We show that path reachability functions can be represented in a
uniform symbolic way as threshold intervals:

\begin{proposition}\label{prop:path:threshold:interval}
  For every nonempty path $\pi$, the family $\{\PPost{\pi}{} :
  \Penab{\pi} \neq \emptyset\}$ is an effective threshold interval of
  size $2 |\pi|$.
\end{proposition}

\begin{proof}
  We give a procedure that proceeds inductively on~$|\pi|$. If $|\pi|
  = 1$, then $\pi$ is a transition $t$. Note that $\effect{t}$ is
  either a constant from $\Q$ or a parameter from $Y$. Since we only
  consider consistent valuations, we know whether $\effect{t}$ is
  strictly negative or postive. Consequently, we can define the
  following negative and positive linear expressions:
  \begin{align*}
    \Psi_{\max} &\defeq
    \begin{cases}
      \effect{t} & \text{if } \effect{t} < 0, \\
      \more{0}   & \text{if } \effect{t} > 0, \\
      0          & \text{otherwise},
    \end{cases} &
    %
    \Psi_{\min} &\defeq
    \begin{cases}
      \effect{t} & \text{if } \effect{t} > 0, \\
      \less{0}   & \text{if } \effect{t} < 0, \\
      0          & \text{otherwise}.
    \end{cases}
  \end{align*}
  We have $\PPost{\pi}{x} = (x + (0, 1] \cdot \effect{t}) \cap
  \guard{\Out{t}}$. Thus, the family $\{\PPost{\pi}{} :
  \Penab{\pi} \neq 0\}$ is representable as this threshold
  interval: \[[\max(x \oplus \Psi_{\max},
    \psi_{\max}),\ \min(x \oplus \Psi_{\min},
    \psi_{\min})],\] where $\psi_{\max} \defeq \inf
  \guard{\Out{t}}$ and $\psi_{\min} \defeq \sup \guard{\Out{t}}$ are
  either constants or parameters.

  If $|\pi| \geq 2$, then $\pi = \sigma t$ for some path $\sigma$ and
  transition $t$. By induction, the families $\{\PPost{\sigma}{} :
  \Penab{\sigma} \neq \emptyset\}$ and $\{\PPost{t}{} : \Penab{t} \neq
  \emptyset\}$ are representable by such threshold intervals:

  \philip{should the right-hand bound say $\min_{\varphi \in E_{\min}} \varphi$
  instead of $\max_{\varphi \in E_{\min}} \varphi$? intuitively, $E_{min}$ corresponds
  to upper guards, and we need to respect all guards, so should be at most the smallest guard, not the largest guard}
  \begin{alignat*}{2}
    & [\max(x \oplus \Phi_{\max}, \max_{\varphi \in E_{\max}} \varphi)),\
    %      
    && \min(x \oplus \Phi_{\min}, \max_{\varphi \in E_{\min}} \varphi)] \\
    %
    & [\underbrace{\max(x \oplus \Psi_{\max},
          \psi_{\max})}_{\ell(x)},\
    %
    && \underbrace{\min(x \oplus \Psi_{\min}, \psi_{\min})}_{h(x)}].
  \end{alignat*}

  \philip{$\ell^\mu$ and $h^\mu$ are used with the superscript, but defined without it here, should
  we mention this explicitly?}
  For all $x \in \Penab{\pi}$, $\PPost{\pi}{x}$ is an interval by
  \autoref{prop:path:interval}. Moreover, functions $\ell^\mu$ and
  $h^\mu$ are monotonic. Thus, we have:
  \begin{alignat*}{2}
    \PPost{\pi}{x}
    %
    &=\ && \PPost{t}{\PPost{\sigma}{x}} \\
    %
    &=\ && [\ell^\mu(\inf \PPost{\sigma}{x}),\
             h^\mu(\sup \PPost{\sigma}{x})] \\
    %
    &=\ && [\max(x \oplus (\Phi_{\max} \oplus \Psi_{\max})^\mu,
      \max_{\varphi \in E_{\max}} (\varphi \oplus \Psi_{\max})^\mu,
      \psi_{\max}^\mu), \\[-2pt]
      %
    &&& \phantom{[} \min(x \oplus (\Phi_{\min} \oplus \Psi_{\min})^\mu,
        \min_{\varphi \in E_{\min}} (\varphi \oplus \Psi_{\min})^\mu,
        \psi_{\min}^\mu)].
  \end{alignat*}

  \philip{to me it seems like in the second step you would want to have this:}
    $[\ell^\mu(\inf \PPost{\sigma}{x} \cap \Penab{t}),\
    h^\mu(\sup \PPost{\sigma}{x} \cap \Penab{t})]$
  \philip{I think it comes out to the same value, since $\Psi_{\max} = \inf \enab{t}$,
  but maybe one should explicitly point this out. 
  It seems like it works, but there is some subtlety that could be mentioned briefly}
  
  Thus, the family $\{\PPost{\pi}{} : \Penab{\pi} \neq \emptyset\}$
  can be represented by:
  \begin{alignat*}{2}
    & [\max(x \oplus (\Phi_{\max} \oplus \Psi_{\max}),
      \max_{\varphi \in E_{\max}} (\varphi \oplus \Psi_{\max}),
      \psi_{\max}), \\[-2pt]
      %
    & \phantom{[} \min(x \oplus (\Phi_{\min} \oplus \Psi_{\min}),
        \min_{\varphi \in E_{\min}} (\varphi \oplus \Psi_{\min}),
        \psi_{\min})].
  \end{alignat*}
  Note that the sum of the two negative linear expressions
  $\Phi_{\max} \oplus \Psi_{\max}$ yields a negative linear
  expression. Similarly, $\Phi_{\min} \oplus \Psi_{\min}$ is positive,
  and the left and right expressions remain left and right. Thus, we
  obtain a threshold interval of size $(|E_{\max}| + 1) + (|E_{\min}|
  + 1) = (|E_{\max}| + |E_{\min}|) + 2 = 2|\sigma| + 2|t| = 2|\pi|$.
\end{proof}

We now show that reachability functions for cycles are representable
in a similar symbolic fashion. The data structure is a slight
adaptation of the one for paths. We define \emph{pseudo-threshold
  intervals} as threshold intervals, but where the two terms $x \oplus
\Psi_{\max}$ and $x \oplus \Psi_{\min}$ are not mandatory, i.e.\ the
endpoints may or may not depend on $x$. Informally, this is due to the
fact that ``accelerating'' a cycle through repeated iterations can
reach all values towards some guard. We define size and effectiveness
of pseudo-threshold intervals in the same way.

\begin{proposition}\label{prop:cycle:threshold:interval}
  For every cycle $\Theta$, $\{\PPost{\Theta^+}{} : \Penab{\Theta^2}
  \neq \emptyset\}$ is an effective pseudo-threshold interval of size
  $2 |\Theta|$.
\end{proposition}

\begin{proof}
  By definition and by \autoref{prop:thetatwo}, we only consider
  consistent valuations $\mu$ with $\Penab{\Theta} = \Penab{\Theta^2}
  = \cdots \neq \emptyset$. Let $\{\PPost{\Theta}{} : \Penab{\Theta}
  \neq \emptyset\}$ be represented by the following threshold interval
  given by \autoref{prop:path:threshold:interval}:
  \begin{align}
    [\max(x \oplus \Psi_{\max}, \max_{\varphi \in E_{\max}} \varphi),\
    %
     \min(x \oplus \Psi_{\min}, \max_{\varphi \in E_{\min}} \varphi)].
    %
    \label{eq:rep:interval}
  \end{align}
  \philip{as before, should the right-hand bound use $\min_{\varphi \in E_{\min}} \varphi)$?}
  We introduce these intermediary functions:
  \begin{align*}
    \ell_i^\mu(x)
    %
    &\defeq \max(x \oplus i \cdot \Psi_{\max}^\mu, \max_{\varphi \in
      E_{\max}, 0 \leq j < i}(\varphi^\mu \oplus j \cdot
    \Psi_{\max}^\mu), \\
    %
    h_i^\mu(x)
    %
    &\defeq \min(x \oplus i \cdot \Psi_{\min}^\mu, \min_{\varphi \in
      E_{\min}, 0 \leq j < i}(\varphi^\mu \oplus j \cdot
    \Psi_{\min}^\mu).
  \end{align*}
  We claim that for every $x \in \Penab{\Theta^i}$ and $i \geq 1$,
  we have:
  \[\PPost{\Theta^i}{x} = [\ell_i^\mu(x),\ h_i^\mu(x)].\]

  First recall that $\Penab{\Theta^i} = \Penab{\Theta}$ for every $i
  \geq 1$. The base case $i = 1$ follows immediately from
  \eqref{eq:rep:interval}. Let $i > 1$. We have $\PPost{\Theta^i}{x} =
  \PPost{\Theta^{i-1}}{\PPost{\Theta}{x}}$. Furthermore, this holds by
  the induction hypothesis: \[\PPost{\Theta^{i-1}}{x} =
  [\ell_{i-1}^\mu(x), h_{i-1}^\mu(x)].\] Recall that
  $\PPost{\Theta^i}{x}$ is an interval by
  \autoref{prop:path:interval}. Moreover, functions $\ell_{i-1}^\mu$
  and $h_{i-1}^\mu$ are monotonic. Hence, the endpoints of interval
  $\PPost{\Theta^i}{x}$ are obtained by evaluating these two functions
  on the endpoints of $\PPost{\Theta}{x}$, i.e.\
  \begin{align*}
    \PPost{\Theta^i}{x}
    %
    &=[\ell_{i-1}^\mu(x \oplus \Psi_{\max}^\mu, \max_{\varphi \in E_{\max}}
      \varphi^\mu),\ h_{i-1}^\mu(x \oplus \Psi_{\min}^\mu, \min_{\varphi
        \in E_{\min}} \varphi^\mu)] \\
    %
    &= [\ell_i^\mu(x), h_i^\mu(x)].
  \end{align*}

  We may now prove the proposition. Let $x \in \Penab{\Theta}$. By
  \autoref{prop:path:interval} and the claim, the following set is an
  interval:
  \[
  \PPost{\Theta^+}{x}
  = \bigcup_{i \geq 1} \PPost{\Theta^i}{x}
  = \bigcup_{i \geq 1}\; [\ell_i^\mu(x), h_i^\mu(x)].
  \]
  Since we have $x \in \Penab{\Theta} = \Penab{\Theta^2} = \cdots$,
  each interval $[\ell_i^\mu(x), h_i^\mu(x)]$ is
  nonempty. Therefore, we have:
  \[
  \PPost{\Theta^+}{x} = [\inf_{i \geq 1} \ell_i^\mu(x), \sup_{i \geq
      1} h_i^\mu(x)].
  \]

  To conclude the proof, we must provide a representation of the two
  above endpoints with linear expressions. Recall that $\Psi_{\max}$
  is a negative linear expression. In particular, this means that
  $\Psi_{\max}^\mu$ belongs to $\cup_{c \in \Q_{\leq 0}} \{c,
  \more{c}\}$. Thus, either $\Psi_{\max}^\mu \in \{0, \more{0}\}$ or
  $\Psi_{\max}^\mu$ is strictly negative. In the former case, we have
  $\ell_1(x) \preceq \ell_2(x) \preceq \cdots$. In the latter case,
  $\inf_{i \geq 1} \ell_i^\mu(x) = \max_{\varphi \in E_{\max}}
  \varphi^\mu$ as the other terms decrease towards
  $-\infty$. Altogether, this yields:
  \[
  \inf_{i \geq 1} \ell_i^\mu(x)
  =
  \begin{cases}
    \ell_1^\mu(x)
    %
    & \text{if $\Psi_{\max}^\mu \in \{0, \more{0}\}$}, \\
    %
    \max_{\varphi \in E_{\max}} \varphi^\mu
    %
    & \text{otherwise}.
    %
  \end{cases}
  \]
  This provides a correct representation w.r.t.\ $\mu$. However, we
  are not entirely done as we should be use the same linear
  expressions for \emph{all} consistent valuations $\mu$. Fortunately,
  this is the case. Indeed, it only depends on the syntactic form of
  $\Psi_{\max}$: the first case above holds if $\Psi_{\max} \in \{0,
  \more{0}\}$, and the second case holds otherwise, so if
  $\Psi_{\max}$ constains a negative constant or at least one
  parameter (which has to be from $Y^{-}$).

  Symmetrically, we have $\sup_{i \geq 1} h_i^\mu(x) = \min_{\varphi
    \in E_{\min}} \varphi^\mu$ if $\Psi_{\min}$ contains at least one
  parameter (which has to be from $Y^{+}$) or a positive constant, and
  $\sup_{i \geq 1} h_i^\mu(x) = h_1^\mu(x)$ otherwise.
\end{proof}

\subsection{\NP-completeness via existential linear arithmetic}

\begin{lemma}\label{lem:path:cycle:formula}
  For every path $\pi$ and every cycle $\Theta$, there are
  polynomial-time computable quantifier-free linear formulas
  $\varphi_\pi$ and $\varphi_{\Theta^+}$ such that if $\mu$ is a
  consistent valuation, then:
  \begin{itemize}
  \item $\varphi_\pi(x, x', \mu)$ holds iff $x \in \Penab{\pi}$ and
    $x' \in \PPost{\pi}{x}$,

  \item $\varphi_{\Theta^+}(x, x', \mu)$ holds iff $x \in
    \Penab{\Theta^2}$ and $x' \in \PPost{\Theta^+}{x}$.
  \end{itemize}
\end{lemma}

\begin{proof}
  First note that membership in (pseudo-)threshold intervals can be
  easily translated into a quantifier-free formula. For example, the
  following constraint:
  \[
  x' \in [\max(x \oplus y_1 \oplus 3 y_2 \oplus (-7), 5 y_1 \oplus
    \more{0}),\ \min(x \oplus \less{0}, 6 y_4 \oplus +\infty)]
  \]
  can be translated into this formula:
  \[
  (x' \geq x + y_1 + 3 y_2 - 7) \land (x' > 5 y_1) \land
  (x' <    x).
  \]
  \michael{TODO. $\mathrm{enab}^\mu(\pi)$ and
    $\mathrm{enab}^\mu(\Theta^2)$ can be encoded the same way via
    unrolling, and $\mathrm{Post}^\mu_\pi$ and
    $\mathrm{Post}^\mu_{\Theta^+}$ can be translated via an encoding
    of (pseudo)-threshold intervals (via
    \autoref{prop:path:threshold:interval} and
    \autoref{prop:cycle:threshold:interval}). Technical detail: the
    latter encoding works due to the fact that we have left
    expressions under $\max$ and right expressions under $\min$.}
\end{proof}

\begin{proposition}\label{prop:flat:param:np}
  The reachability problem for flat parametric COCAs belongs in \NP.
\end{proposition}

\begin{proof}
  Let $\Pp = (Q, T, \tau, Y)$ be a parametric COCA, let $\Lambda$ be a
  linear path scheme of $\Pp$, and let $x, x' \in \Q$ be values for
  which we wish to verify that $x' \in \Post{\Lambda}{x}$. For each
  cycle $\Theta$ of $\Lambda$, we guess whether $\Theta$ will be used
  zero, once or several times. In the first case, we simply remove
  $\Theta$; in the second one, we replace $\Theta^*$ by the path
  $\Theta$; and in the third one, we replace $\Theta^*$ by
  $\Theta^+$. Let $\Lambda' = \pi_0 \Theta_1^+ \pi_1 \cdots \Theta_n^+
  \pi_n$ be the resulting expression.

  We further nondeterministically partition $Y$ into parameters that
  must be strictly negative, strictly positive, or equal to
  zero. Parameters of the latter kind are simply replaced by $0$
  within $\Pp$. Hence, the remaining parameters are partitioned into
  sets $Y^{-}$ and $Y^{+}$. Using \autoref{lem:path:cycle:formula}, we
  construct in polynomial time this sentence $\Psi$ of the existential
  fragment of linear arithmetic:
  \begin{align*}
    &\exists \mu \in \Q^Y
    \exists x_0, x_0' \ldots, x_n, x_n' \in \Q : 
    %
    \bigwedge_{y \in Y^{-}} \mu(y) < 0 \land
    \bigwedge_{y \in Y^{+}} \mu(y) > 0 \land {} \\[-2pt]
    %
    &
    (x_0 = x) \land
    \bigwedge_{0 \leq i \leq n} \varphi_{\pi_i}(x_i, x_i', \mu) \land
    \bigwedge_{0 < i \leq n} \varphi_{\Theta_i^+}(x_{i-1}', x_i, \mu) \land
    (x_n' = x').
  \end{align*}
  In words, $\Phi$ guesses a consistent valuation $\mu$ and
  intermediate values that witness $x' \in \PPost{\Lambda'}{x}$. Since
  determining whether $\Phi$ holds can be achieved in
  \NP~\cite{Son85}, we are done.
\end{proof}

\begin{theorem}
  The reachability problem for flat parametric COCAs belongs is
  \NP-complete, regardless of whether parameters occur on transitions,
  guards or both.
\end{theorem}

\begin{proof}
  Membership in \NP{} has already been established in
  \autoref{prop:flat:param:np}, with no restriction on the
  parameters. Thus, it remains to show \NP-hardness for the cases
  where parameters either only occur on transition or only occur on
  guards.
  In both cases, we give a reduction from 3-SAT.
  Let $\varphi = \bigwedge_{1 \leq j
  \leq m} C_j$ be a 3-CNF formula over variables $X = \{x_1, \ldots,
  x_n\}$. 
  
  Now, let us give two parametric COCA's $\Pp$ and $\Pp'$, both with parameters $X$.
  Each COCA will guess an assignment to it's parameters, and check whether they satisfy
  $\varphi$.
  Additionally, $\Pp$ uses parameters only on guards, and $\Pp'$ uses parameters only on updates.

  \begin{figure}[!h]
    \begin{center}
      \input{fig-np-complete-guessing}
    \end{center}
    \caption{Gadget for variable $x_i$, used in the reduction from 3-SAT to parametric COCA
      reachability. \emph{Left}: Parameters occur only on guards;
      \emph{Right}: Parameters occur only on updates.}
    \label{fig:np:complete-guessing}
  \end{figure}

  \begin{figure}[!h]
    \begin{center}
      \input{fig-np-complete-checking}
    \end{center}
    \caption{Gadgets for clause $C_j = (x_1 \lor x_2 \lor \neg
    x_4)$, used for the reduction from 3-SAT to parametric COCA
      reachability. \emph{Top}: Parameters occur only on guards;
      \emph{Bottom}: Parameters occur only on updates.}
    \label{fig:np:complete-checking}
  \end{figure}

  The first part is achieved by sequentially composing $n$ copies of one of the gadgets depicted
  in \autoref{fig:np:complete-guessing}. The gadget on the left is used by $\Pp$, while
  the gadget on the right is used by $\Pp'$. Both gadgets function in the same manner:
  (1)~state $p_i$ is entered with counter value $0$; (2)~the counter is set to $x_i$; (3)~the counter value is checked to belong to $\{0,1\}$; and (4)~the counter value
  is reset to zero upon leaving to state $q_i$.
  Thus, the only way to traverse the chain of
  $n$ such gadgets from $p_1$ to $q_n$ is to have $x_i \in \{0, 1\}$
  for each $x_i \in X$.

  The second part is achieved by chaining a gadget for each clause
  similar to the one depicted in
  \autoref{fig:np:complete-checking} for $C_j = (x_1 \lor x_2 \lor \neg
  x_4)$. The top gadget is used by $\Pp$, while the bottom gadget is used by $\Pp'$.
  In words, the gadget (1)~enters state $r_j$ with the counter value set to $0$;
  (2)~nondeterministically picks a variable $x_i$ of some
  literal of $C_j$ and increments the counter by $x_i$; (3)~checks
  whether the counter holds the right value w.r.t.\ the literal
  polarity; and (4)~resets the counter to zero upon leaving to state
  $s_j$. Thus, the chain of gadgets can be traversed from $r_1$ to
  $s_m$ iff $\varphi$ is satisfied by the assignment.

  Altogether the following three statements are equivalent:
  (1)~formula $\varphi$ is satisfiable; (2)~there exists a
  valuation $\mu \colon X \to \Q$ such that $p_1(0) \steps{*} s_m(0)$
  holds in $\Pp^\mu$; and (3)~there exists a
  valuation $\mu' \colon X \to \Q$ such that $p_1(0) \steps{*} s_m(0)$
  holds in $\Pp'^{\mu'}$
\end{proof}

\begin{proposition}
  Parametric COCA reachability is \NP-hard.
\end{proposition}

\begin{proof}
  We give a reduction from 3-SAT. Let $\varphi = \bigwedge_{1 \leq j
    \leq m} C_j$ be a 3-CNF formula over variables $X = \{x_1, \ldots,
  x_n\}$. We construct a parametric COCA $\Pp$ with parameters $X$
  that guesses an assignment to $X$ and checks whether it satisfies
  $\varphi$.

  The first part is achieved by sequentially composing $n$ copies of
  the gadget depicted on the left of \autoref{fig:np:complete}. In
  words, it (1)~enters state $p_i$ with the counter set to zero;
  (2)~increments the counter by $x_i$; (3)~checks whether the counter
  value belongs to $\{0, 1\}$; and (4)~resets the counter to zero upon
  leaving to state $q_i$. Thus, the only way to traverse the chain of
  $n$ such gadgets from $p_1$ to $q_n$ is to have $x_i \in \{0, 1\}$
  for each $x_i \in X$.

  The second part is achieved by chaining a gadget for each clause
  similar to the one depicted on the right of
  \autoref{fig:np:complete} for $C_j = (x_1 \lor x_2 \lor \neg
  x_4)$. In words, it (1)~enters state $r_j$ with the counter set to
  zero; (2)~nondeterministically picks a variable $x_i$ of some
  literal of $C_j$ and increments the counter by $x_i$; (3)~checks
  whether the counter holds the right value w.r.t.\ the literal
  polarity; and (4)~resets the counter to zero upon leaving to state
  $s_j$. Thus, the chain of gadgets can be traversed from $r_1$ to
  $s_m$ iff $\varphi$ is satisfied by the assignment.

  Altogether, formula $\varphi$ is satisfiable iff there exists a
  valuation $\mu \colon X \to \Q$ such that $p_1(0) \steps{*} s_m(0)$
  holds in $\Pp^\mu$.
\end{proof}

==> linearps.tex <==
\subsection{Linear case}\label{subsec:lps}

Let us fix a guarded COCA $\W = (Q, T, \tau)$.

\begin{lemma}\label{lem:convex}\label{lemma:convex}
  Let $\pi$ be a path, let $a, a', b, b' \in \Q$ and let $\Lambda \in
    (0, 1]$. If $a \steps{\pi} a'$ and $b \steps{\pi} b'$, then $(1 -
    \Lambda) a + \Lambda b \steps{\pi} (1 - \Lambda) a' + \Lambda b'$.
\end{lemma}

\begin{proof}
  We prove the case where $\pi$ is a transition $t$. The general case
  follows by induction. By definition, there exist $\alpha, \beta \in
    (0, 1]$ such that $a \steps{\alpha t} a'$ and $b \steps{\beta t}
    b'$. Let $\gamma \defeq (1 - \Lambda) \alpha + \Lambda
    \gamma$. Clearly, $\gamma \in (0, 1]$ by convexity and since $(0,
    1]$ is an interval. Hence, we are done since:
  \begin{alignat*}{2}
        & [(1 - \Lambda) a + \Lambda b] + \gamma \Effect{t}                           \\
    %
    =\  & [(1 - \Lambda) a + \Lambda b] + [(1 - \Lambda) \alpha +
    \Lambda \beta] \Effect{t}                                                         \\
    %
    =\  & (1 - \Lambda)(a + \alpha \Effect{t}) + \Lambda (b + \beta
    \Effect{t})                                                                       \\
    %
    =\  & (1 - \Lambda) a' + \Lambda b'.                            & \tag*{\qedhere}
  \end{alignat*}
\end{proof}

\begin{lemma}\label{lemma:enab-interval}\label{lemma:post-intervals}
  For every path $\pi$ and every interval $J \in \intervals$, the
  sets $\enab{\pi}$ and $\Post{\pi}{J}$ are intervals.
\end{lemma}

\begin{proof}
  Assume that $|\enab{\pi}| > 1$, as we are otherwise done. Let $a, c
    \in \enab{\pi}$ be such that $a < c$. We show that any $b \in (a,
    c)$ belongs to $\enab{\pi}$. By definition, $a \steps{\pi} a'$ and
  $c \steps{\pi} c'$ for some $a', c' \in \Q$. We can write $b$ as a
  convex combination of $a$ and $c$, \ie\ $b = (1 - \Lambda) a +
    \Lambda c$ for some $\Lambda \in (0, 1)$. By \autoref{lem:convex},
  we have $b \steps{\pi} (1 - \Lambda) a' + \Lambda c'$, and hence $b
    \in \enab{\pi}$.

  Assume $|\Post{\pi}{J}| > 1$, as we are otherwise done. Let $a', c'
    \in \Post{\pi}{J}$ be such that $a' < c'$. We show that any $b' \in
    (a', c'$) belongs to $\Post{\pi}{J}$. Let $I \defeq J \cap
  \enab{\pi}$, which is an interval by the above. We have $a
  \steps{\pi} a'$ and $c \steps{\pi} c'$ for some $a, c \in
  I$. Moreover, $b' = (1 - \Lambda) a' + \Lambda c'$ for some $\Lambda
  \in (0, 1)$. Let $b \defeq (1 - \Lambda) a + \Lambda c$. By
    \autoref{lem:convex}, we have $b \steps{\pi} b'$ and hence $b' \in
  \Post{\pi}{J}$. Furthermore, $b \in I$ since $I$ is an interval.
\end{proof}

%% Former proof of lemma:enab-interval
%%
%% \begin{proof}
%%   We assume that $\enab{\pi} > 1$, as we are otherwise done. Let $a,
%%   c \in \enab{\pi}$ be such that $a < c$. We must show that any value
%%   $b \in (a, c)$ belongs to $\enab{\pi}$. By definition of $\enab{\pi}$, there exist
%%   runs $\rho, \rho'$ and values $a', c' \in \Q $ such that $a
%%   \steps{\rho} a'$, $c \steps{\rho'} c'$ and $\upath{\rho} = \upath{\rho'}
%%   = \pi$.
%%
%%   Assume that $\rho$ is not admissible from $b$, as we are otherwise
%%   done. Let $a_i \defeq a + \Effect{\FromTo{\rho}{1}{i}}$, $b_i \defeq
%%   b + \Effect{\FromTo{\rho}{1}{i}}$ and $c_i \defeq c +
%%   \Effect{\FromTo{\rho'}{1}{i}}$. Let $j$ be the minimal index such
%%   that $\FromTo{\rho}{1}{j}$ is not admissible from $b$. Let $q \defeq
%%   \Out{\FromTo{\pi}{1}{j}}$. Note that $b_j > a_j$. Thus, $b_j \in
%%   \botguard{q}$ and hence $b_j \not\in \topguard{q}$. Since $c_j \in
%%   \topguard{q}$, this means that $b_j > c_j$.
%%
%%   Let $\sigma' \defeq \FromTo{\rho}{1}{j}$ and $\sigma'' \defeq
%%   \FromTo{\rho}{j+1}{|\sigma|}$. By the above, we have $b < c$, $b_j
%%   > c_j$, $b \steps{\sigma'} b_j$ and $c \steps{\sigma'} c_j$. By
%%   \autoref{lemma:follower}, we obtain $b \steps{\sigma'} c_j$ and
%%   hence $b \steps{\sigma'} c_j \steps{\sigma''} c$. Thus, $b
%%   \steps{\sigma} c$.
%% \end{proof}




% \begin{lemma}
%   Let $t$ be a transition of a guarded COCA, and let $a, b \in \guard{\In{t}}$
%   such that $b \in \enab{t}$ and $a \steps{t} b$.
%   It is the case that $b \in \cl{\Post{t}{b}}$.
% \end{lemma}

% \begin{lemma}
%   Let $t$ be a transition of a guarded COCA, and let $a, b \in \guard{\In{t}}$
%   such that $b \in \enab{t}$ and $a \steps{t} b$.
%   It is the case that $b \in \cl{\Post{t}{b}}$.
% \end{lemma}
% \begin{proof}
%   It must hold that $b \steps{\beta t} b'$ for some $b' \in \guard{\Out{t}}$ and $\beta \in \QZeroOne$, since $b \in \enab{t}$.
%   Further, from $a \steps{t} b$ it follows that $a \steps{\alpha t} b$ for some $\alpha \in \QZeroOne$.

%   Let us first note that it must hold that either $a = b = b'$ (if $\Effect{t} = 0$), $a < b$ and $b < b'$ (if $\Effect{t} > 0$), or $a > b$ and $b > b'$ (if $\Effect{t} < 0$).
%   In case $a = b = b'$, we are done. So assume one of the other cases holds.
%   Without loss of generality, let us assume $\Effect{t} > 0$, so $a < b$ and $b < b'$; the other case will follow by symmetry.

%   To show that $\cl{\Post{t}{b}}$, it suffices to show that $b + \varepsilon \in \cl{\Post{t}{b}}$ for all $0 < \varepsilon < 1$.
%   Let $\beta = \dfrac{\varepsilon}{\abs{\Effect{t}}}$. Since we allow effects of transitions to be integers, and $\varepsilon < 1$, it holds that $\beta \in \QZeroOne$. Note that $b + \beta \Effect{t} = b +  \dfrac{\varepsilon}{\abs{\Effect{t}}} \Effect{t} = b + \varepsilon$. Lastly, note that $b < b + \varepsilon < b'$, and $b, b' \in \guard{\Out{t}}$, so $b + \varepsilon \in \guard{\Out{t}}$. It follows that $b \steps{\beta t} b + \varepsilon$, so $b + \varepsilon \in \Post{t}{b}$, so $b \in \cl{\Post{t}{b}}$.
% \end{proof}


\begin{lemma}\label{lemma:follower}
  Let $t \in T$, $\alpha, \beta \in (0, 1]$ and $a, a', b, b' \in \Q$
    be such that $a' = a + \alpha \Effect{t}$ and $b' = b + \beta
    \Effect{t}$. If $a \leq b$ and $a' \geq b'$, then $b' = a +
    \alpha' \Effect{t}$ and $a' = b + \beta' \Effect{t}$ for some
    $\alpha', \beta' \in (0, 1]$.
\end{lemma}

\begin{proof}
  The claim is trivial whenever $a = b$ or $a' = b'$, hence assume $a
  < b$ and $a' > b'$. Note that $\Effect{t} \neq 0$, as we would
  otherwise derive the contradiction $a < b = b' < a' = a$. Let
  \[
    \alpha' \defeq \dfrac{b' - a}{\Effect{t}} \text{ and }
    %
    \beta' \defeq \dfrac{a' - b}{\Effect{t}}.
  \]
  We have $a + \alpha' \Effect{t} = b'$ and $b + \beta' \Effect{t} =
  a'$ as desired. It remains to show that $\alpha', \beta' \in (0,
  1]$. From $a' > b'$, we have:
  \begin{alignat*}{4}
    \alpha'
    &=\ & (b' - a) / \Effect{t}
    &<\ & (a' - a) / \Effect{t}
    &=\ & \alpha \leq 1, \\
    %
    \beta'
    &=\ & (a' - b) / \Effect{t}
    &>\ & (b' - b) / \Effect{t}
    &=\ & \beta > 0.
  \end{alignat*}
  From $a < b$, we symmetrically derive $\alpha' > 0$ and $\beta' \leq
  1$.
\end{proof}

%% Old broken Lemma 9
%% \begin{lemma}\label{lemma:follower}
%%   Let $a, a', b, b' \in \Q$ be such that $a < b$ and $a' > b'$. If $a
%%     \steps{\pi} a'$ and $b \steps{\pi} b'$, then $a \steps{\pi} b'$
%%   and $b \steps{\pi} a'$.
%% \end{lemma}

%% \philip{I think we need a version of this lemma where we don't reason about runs,
%%   but pseudoruns - again, usually one would want to use this
%%   when $b \steps{\pi} b'$ is precisely not a run,
%%   but then $b \steps{\pi} a'$ is.}

%% \begin{proof}
%%   By assumption, there exist runs $\rho, \rho'$ such that $a \steps{\rho}
%%     a'$, $b \steps{\rho'} b'$ and $\upath{\rho} = \upath{\rho'} = \pi$.
%%   Let $a_i \defeq a + \Effect{\FromTo{\rho}{1}{i}}$ and $b_i \defeq b +
%%     \Effect{\FromTo{\rho'}{1}{i}}$. Let $j$ be the maximal index such that
%%   $a_j < b_j$. Let $n \defeq |\pi|$. Note that $j < n$ as $a' >
%%     b'$. Let $t \defeq \pi_{j+1}$, \ie\ the $(j+1)$-th transition used
%%   by both runs. It suffices to show that $a_j \steps{t} b_{j+1}$ and
%%   $b_j \steps{t} a_{j+1}$ since it yields:
%%   \begin{align*}
%%      &
%%     a       \steps{\FromTo{\rho}{1}{j}}
%%     a_j     \steps{t}
%%     b_{j+1} \steps{\FromTo{\rho'}{j+2}{n}}
%%     b', \\
%%     %
%%      &
%%     b       \steps{\FromTo{\rho'}{1}{j}}
%%     b_j     \steps{t}
%%     a_{j+1} \steps{\FromTo{\rho}{j+2}{n}}
%%     a'.
%%   \end{align*}

%%   Let us prove this claim. If $a_{j+1} = b_{j+1}$, then we are
%%   done. Otherwise, we have $a_{j+1} > b_{j+1}$ by maximality of
%%   $j$. Note that $\Effect{t} \neq 0$, as we would otherwise derive the
%%   contradiction $a_j < b_j = b_{j+1} < a_{j+1} = a_j$. By definition,
%%   there exist $\alpha, \beta \in (0, 1]$ such that $a_j + \alpha
%%     \Effect{t} = a_{j+1}$ and $b_j + \beta \Effect{t} = b_{j+1}$. Let
%%   \[
%%     \alpha' \defeq \dfrac{b_{j+1} - a_j}{\Effect{t}} \text{ and }
%%     %
%%     \beta' \defeq \dfrac{a_{j+1} - b_j}{\Effect{t}}.
%%   \]
%%   We have $a_j + \alpha' \Effect{t} = a_j + [(b_{j+1} - a_j) /
%%     \Effect{t}] \cdot \Effect{t} = b_{j+1}$ and $b_j + \beta'
%%     \Effect{t} = b_j + [(a_{j+1} - b_j) /\Effect{t}] \cdot \Effect{t} =
%%     a_{j+1}$ as desired.

%%   It remains to show that $\alpha', \beta' \in (0, 1]$. It follows
%%   from $a_{j+1} > b_{j+1}$ that $\alpha' = (b_{j+1} - a_j) /
%%     \Effect{t} < (a_{j+1} - a_j) / \Effect{t} = \alpha \leq 1$. and
%%   $\beta' = (a_{j+1} - b_j) / \Effect{t} > (b_{j+1} - b_j) /
%%     \Effect{t} = \beta > 0$. From $a_j < b_j$, we symmetrically derive
%%   $\alpha' > 0$ and $\beta' \leq 1$.
%% \end{proof}


%% Not needed
%%
%% \begin{lemma}
%%   Let $\pi$ be a path and let $a, b \in \Q$. If $a \steps{\pi} b$
%%   and $b \in \enab{\pi}$, then $b \in \cl{\Post{\pi}{b}}$.
%% \end{lemma}

%% \begin{proof}
%%   We assume that $b \not\in \Post{\pi}{b}$, as we are otherwise
%%   done. By definition, there exist a run $\rho$ and a value $c \in \Q$
%%   such that $b \steps{\rho} c$. Let us consider the case where $c >
%%     b$. The case $c < b$ is symmetric. We must show that any $b' \in (b,
%%     c)$ can be reached from $b$ via path $\pi$. Let $\beta \defeq (b' -
%%     b) / (c - b)$ and $\rho' \defeq \beta \rho$. Clearly, $\beta \in (0,
%%     1]$. Moreover, $b + \Effect{\rho'} = b + \beta (c - b) = b + (b' - b)
%%     = b'$. Hence, if run $\rho'$ is admissible from $b$, then we are
%%   done.

%%   For the sake of contradiction, suppose it is not. By assumption,
%%   there exists a run $\sigma$ such that $a \steps{\sigma} b$ and
%%   $\upath{\sigma} = \pi$. Let $a_i \defeq a +
%%     \Effect{\FromTo{\sigma}{1}{i}}$, $b_i \defeq b +
%%     \Effect{\FromTo{\rho}{1}{i}}$ and $b_i' \defeq b +
%%     \Effect{\FromTo{\rho'}{1}{i}}$, $q_i \defeq \Out{\pi_i}$ and $n
%%     \defeq |\rho'|$. Clearly, $b_i' \leq b_i$ and hence $b_i' \in
%%     \topguard{q_i}$ for every $1 \leq i \leq n$. Thus, $\rho'$ is not
%%   admissible from $b$ because it violates a lower guard. Since
%%   $\sigma$ is admissible from $a$, there is a minimal $j < n$ such
%%   that $b_j' \geq a_j$ and $b_{j+1}' < a_{j+1}$. If $b_j' = a_j$, then
%%   $b \steps{\FromTo{\rho'}{1}{j}} a_{j} \steps{\FromTo{\sigma}{j+1}{n}}
%%     b$, which is a contradiction. If $b_j' > a_j$, then
%%   \autoref{lemma:follower} yields $b_j' \steps{\pi_{j+1}} a_{j+1}$
%%   and hence a contradiction:
%%   \[
%%     b       \steps{\FromTo{\rho'}{1}{j}}
%%     b'_j    \steps{\pi_{j+1}}
%%     a_{j+1} \steps{\FromTo{\sigma}{j+2}{n}}
%%     b. \qedhere
%%   \]
%% \end{proof}

%% \begin{lemma}
%%   Let $\pi$ be a path of a guarded COCA, and let $a, b \in \guard{\In{\pi}}$ such that $b \in \enab{\pi}$ and $a \steps{\pi} b$.
%%   Then $b \in \cl{\Post{\pi}{b}}$.
%% \end{lemma}

%% \begin{proof}
%%   By the definition of $\enab{\pi}$, there must exist some $b' \in \guard{\Out{\pi}}$ and a run $\rho$ with $\upath{\rho} = \pi$ such that $b \steps{\rho} b'$.

%%   Additionally, there must be a run $\sigma$ with $\upath{\sigma} = \pi$ 
%%   such that $a \steps{\sigma} b$, since $a \steps{\pi} b$.

%%   Let us make a case distinction based on the order of $a, b$ and $b'$.

%%   Note that if $a = b$ or $b = b'$, we are done. So let us handle the remaining cases.

%%   If $a < b$ and $b > b'$ or $a > b$ and $b < b'$, by generalizing \autoref{lemma:follower} to sequences of transitions we can follow that $b \steps{\pi} b$, so we are done.

%%   For the last case, let us assume without loss of generality that $a < b < b'$;
%%   the case $a > b > b'$ follows by symmetry.

%%   We aim to show that $b \in \cl{\Post{\pi}{b}}$. To do so, we show that for all $\varepsilon$ such that $0 < \varepsilon < b' - b$, it holds that $\omega \in \cl{\Post{\pi}{b}}$ with $b \leq \omega \leq b + \varepsilon$. First, let us note that $b < b + \varepsilon \leq b'$. Since $b, b' \in \guard{\Out{\pi}}$, it follows that $b + \varepsilon \in \guard{\Out{\pi}}$.

%%   Let us write $\pi = t_1 \dots t_n$ for some $t_1 \dots t_n$. Then let us write $\rho = \gamma_1 t_1 \dots \gamma_n t_n$ for some $\gamma_1, \dots, \gamma_n \in \QZeroOne$.

%%   Let us define $\beta = \dfrac{\varepsilon}{b' - b}$. It holds that $\beta \in \QZeroOne$ by the fact that $\varepsilon < b' - b$ and $b' > b$.
%%   We claim that $\beta \rho$ is a run from $b$ to $b + \varepsilon$ (but we do not claim that this run is admissible).
%%   It suffices to observe that $b + \Effect{\beta \rho} = b + \beta \Effect{\rho} = b + \dfrac{\varepsilon}{b' - b} (b' - b) = b+\varepsilon$. So $\beta \rho$ has the right effect to reach $b + \varepsilon$ from $b$.
%%   In case $\beta \rho$ is admissible from $b$, it immediately follows that $b \steps{\pi} b + \varepsilon$. So let us assume that $\beta \rho$ is not admissible.

%%   Then for some $i$, it must hold that $b + \Effect{\FromTo{\beta\rho}{1}{i}} \notin \guard{\Out{\FromTo{\rho}{1}{i}}}$.
%%   Note that since $\beta \leq 1$ and $\rho$ is admissible from $\beta$, it holds that $\topguard{\Out{\FromTo{\rho}{1}{i}}} \geq b + \Effect{\FromTo{\rho}{1}{i}} \geq b + \Effect{\FromTo{\beta \rho}{1}{i}}$.
%%   So it must be the case that $b + \Effect{\FromTo{\beta\rho}{1}{i}} < \botguard{\Out{\FromTo{\rho}{1}{i}}}$.
%%   Observe that $\sigma$ is admissible from $a$. Therefore, it must hold that $a + \Effect{\FromTo{\sigma}{1}{i}} \geq \botguard{\Out{\FromTo{\rho}{1}{i}}}$. Therefore, $a + \Effect{\FromTo{\sigma}{1}{i}} > b + \Effect{\FromTo{\beta\rho}{1}{i}}$. By assumption, also  $a < b$. Then by \autoref{lemma:follower}, there exists some run $\phi$ with $\upath{\phi} = \pi$ and $b \steps{\phi} a + \Effect{\FromTo{\sigma}{1}{i}}$. Then $b \steps{\phi\FromTo{\sigma}{i+1}{n}} b$.

%%   \philip{this needs one- or two-(hundred) refinements, but technically seems ok}
%% \end{proof}

\begin{lemma}\label{lemma:postplus_interval}
  Let $\mathcal{J}$ be a finite union of intervals and let $\pi$ be a
  cycle. If $\effect{t} \neq 0$ for some $t \in \pi$, then
  $\Post{\pi^+}{\mathcal{J}}$ is an interval.
\end{lemma}

%%% 1st attempt...
% \begin{proof}
%   Without loss of generality, let us assume $\mathcal{J} = J_1 \cup J_2 \dots J_n$ 
%   where each $J_i$ is an interval, and such that $\sup(J_{i}) < \inf(J_{i+1})$ for all $i < n$.
%   By the assumption that $\mathcal{J}$ is a finite union of intervals, such a factorization exists.

%   \philip{Factorization seems like the right word here, but I am unsure}

%   We set $\mathcal{I}_i = \Post{\pi^i}{\mathcal{J}}$.
%   In particular, $\mathcal{I_0} =  \Post{\pi^0}(\mathcal{J}) = \mathcal{J}$.

%   For all $i$, let $n_i$ be the smallest number such that $mathcal{I}_i$ is the union of $n_i$ intervals. Note that $n_i \leq n_{i-1}$ by \autoref{lemma:post-intervals}, since each of the $n_{i-1}$ intervals in $mathcal{I}_{i-1}$ will result in at most one interval in $mathcal{I}_{i}$. Note that since some of these intervals may overlap, it is not necessarily the case that $n_i = n_{i-1}$.

%   Let us assume a factorization $mathcal{I}_i = I_1 \dots I_{n_i}$  such that  $\sup(I_{j}) < \inf(I_{j+1})$ for all $j < n_{i}$. As for $\mathcal{J}$, $\mathcal{I}_i$ must be a finite union of intervals, so such a factorization exists. Additionally, this factorization is uniquely determined by the fact that we require $\sup(I_{j}) < \inf(I_{j+1})$.
%   Let $d_i$ be the largest gap between two neighboring intervals of $I$, that is, we define $d_i = 0$ if $n_{i} = 1$, otherwise $d_i = max_{j < n_{i}}(\inf(I_{j+1}) - \sup(I_{j})$. Observe that $d_i \geq 0$ by the fact that we assume the factorization of $\mathcal{I}_i$ is ordered.

%   We show that for all $i \geq 0$, $d_{i} = d_{i+1} = 0$ or $d_{i} > d_{i+1}$.

%   It is clear that by definition, for all $i$ $d_{i} \geq 0$.
%   Recall that $d_{i} = 0$ means that $mathcal{I}_i$ is a single interval. Then by \autoref{lemma:post-intervals}, $mathcal{I}_{i+1}$ is a single interval, so $d_{i+1} = 0$. 

%   So let us assume that $d_{i} > 0$, then we need to show that $d_{i} > d_{i+1}$.
%   Let us take $j$ such that $d_{i} = \inf(I_{j}) - \inf(I_{j-1})$, where we factor $mathcal{I}_i = I_1 \dots I_{n_i}$ with  $\sup(I_{j}) < \inf(I_{j+1})$ for all $j < n_{i}$, as before.
%   So $I_{j}$ and $I_{j-1}$ are neighboring intervals with a largest gap between them.

%   By definition of $\mathcal{I}_{i+1}$, 
%   \philip{TODO: remember to continue this proof}
% \end{proof}

%%% 3rd attempt
\begin{proof}
  Assume that $|\Post{\pi^+}{\mathcal{J}}| > 1$, as we are otherwise
  done. Let $a', c' \in \Post{\pi^+}{\mathcal{J}}$ be such that $a' <
  c'$. We must show that any $b' \in (a', c')$ belongs to
  $\Post{\pi^+}{J}$. By definition, there exist values $a, b \in
  \mathcal{J}$ and runs $\sigma, \rho$ such that $a \steps{\sigma} a'$,
  $c \steps{\rho} c'$ and $\upath{\sigma}, \upath{\rho} \in \pi^+$. Let
  $\rho = \alpha_1 t_1 \cdots \alpha_n t_n$. Suppose that $\effect{t}
  < 0$ for some $t \in \pi$. The positive case is symmetric.

  We assume $c \neq b'$ as we are otherwise done. Let us construct a
  run $\phi$ such that $\upath{\phi} \in \pi^+$ and $\Effect{\phi} =
  b' - c$. If $b' > c$, then we can take $\phi \defeq \beta \rho$ for a
  suitable $\beta \in (0, 1]$ since $\Effect{\rho} = c' - c > b' -
    c$. If $b' < c$, then we first rescale $\rho$ into a run $\rho'$
    with negative effect. Formally, let $\rho' \defeq \alpha_1' t_1
    \cdots \alpha_n' t_n$ where
  \[
  \alpha_i' \defeq
  \begin{cases}
    1 / (2n \cdot \Effect{t_i})
    & \text{if $\Effect{t_i} > 0$}, \\
    %
    1
    & \text{otherwise}.
  \end{cases}
  \]
  We have $\Effect{\rho'} \leq 1/2 - 1 = -1/2$ and hence
  $\Effect{\beta \rho'} = -1/2$ for some $\beta \in (0, 1]$. Let $\phi
  \defeq (\beta \rho')^{2(c - b')}$. We have $\effect{\phi} = b' -
  c$.

  If run $\phi$ is admissible from $c$, then we are done as we obtain
  $c \steps{\phi} b'$. Otherwise, let $a_i \defeq a +
  \Effect{\FromTo{\sigma}{1}{i}}$, $b_i \defeq c +
  \Effect{\FromTo{\phi}{1}{i}}$ and $c_i \defeq c +
  \Effect{\FromTo{\rho}{1}{i}}$. There exists a maximal $j < |\phi|$
  such that one of these two cases holds: $b_j \not\in
  \botguard{\Out{\phi_j}}$ or $b_j \not\in \topguard{\Out{\phi_j}}$.

  \begin{figure}
    \begin{center}
      \input{fig-interval-merge}
    \end{center}
    \caption{\emph{Gray blocks}: guards; \emph{solid black}: runs $a
      \steps{\sigma} a'$ and $c \steps{\rho} c'$; \emph{dashed red}:
      inadmissible run $\phi$ from $c$ to $b'$; \emph{filled blue}:
      combined run $a \steps{\pi^+} b'$.}%
    \label{fig:interval:merge}
  \end{figure}

  \emph{Case 1:} Although $\phi$ and $\sigma$ may not have the same
  length, they both use $\pi$. So, each nonfinal state of $\phi$ has
  (at least) one counterpart in $\sigma$ with the same outgoing
  transition. Formally, for each $i < |\phi|$, there is some $f(i) <
  |\sigma|$ with $\phi_{i+1} = \sigma_{f(i)+1}$. Since $\sigma$ is
  admissible from $a$, there is a maximal $\ell$ such that $j \leq
  \ell < |\phi|$ and $b_\ell < a_{f(\ell)}$. In particular,
  $b_{\ell+1} \geq a_{f(\ell)+1}$. Thus, we may combine the two runs
  with \autoref{lemma:follower} (see~\autoref{fig:interval:merge}):
  \[
  a \steps{\FromTo{\sigma}{1}{f(\ell)}} a_{f(\ell)}
  \steps{\sigma_{f(\ell) + 1}} b_{\ell+1}
  \steps{\FromTo{\phi}{\ell+2}{|\phi|}} b'.
  \]
  \emph{Case 2:} It is symmetric. More precisely, we define $f$
  w.r.t.\ $\rho$, take $\ell \geq j$ such that $b_\ell > c_{f(\ell)}$
  and $b_{\ell+1} \leq c_{f(\ell)+1}$, and obtain:
  \[
  c \steps{\FromTo{\rho}{1}{f(\ell)}} c_{f(\ell)} \steps{\rho_{f(\ell) +
      1}} b_{\ell+1} \steps{\FromTo{\phi}{\ell+2}{|\phi|}}
  b'. \qedhere
  \]
\end{proof}

%% %%% 2nd attempt...
%% \begin{proof}
%%   Let $n = \abs{\pi}$, then we write $\pi = t_1 \dots t_n$.
%%   We assume that for some $i$, $\effect{t_i} < 0$.
%%   The case $\effect{t_i} > 0$ is symmetric.
%%   Let us define $I = \mathcal{J} \cap \guard{\In{\pi}}$,
%%   $I' = \guard{\Out{\pi}}$.
%%   Assume we have $a', c' \in I'$ such that $a' < c'$, and
%%   $a, c \in I$ such that $a \steps{\pi^{+}} a'$, $c \steps{\pi^+} c'$,
%%   that is, $a' \in \Post{\pi^+}{a}$ and $c' \in \Post{\pi^+}{c}$.
%%   Note that from \autoref{lemma:follower},
%%   we can assume without loss of generality that $a \leq c$.

%%   Our goal is to show that for any $b' \in \Q$ such that $a' < b' < c'$,
%%   it holds that $b' \in \Post{\pi^+}{J}$.
%%   Let $a \in \Post{\pi^*}{\mathcal{J}}$ be such that $a \steps{\pi} a'$ and
%%   $c \in \Post{\pi^*}{\mathcal{J}}$ be such that $c \steps{\pi} c'$.
%%   By definition, there exist runs $\rho, \sigma$ such that $a \steps{\rho} a'$
%%   and $c \steps{\sigma} c'$.

%%   Let us set $b = b' + 0.5$.
%%   We define $\Lambda_+ = \Sigma_{t \in \pi} max(0, \Effect{t})$
%%   and $\Lambda_- = \Sigma_{t \in \pi} min(0, \Effect{t})$.
%%   In particular, note that $\Lambda_+ + \Lambda_- = \Effect{\pi}$.
%%   Now, let us define for all $1 \leq i \leq n$ that
%%   \begin{gather*}
%%     \beta_i = \begin{cases}
%%       \dfrac{-1}{\Lambda_-}  & \text{if $\Effect{t_i} \leq 0$, and} \\
%%       \dfrac{0.5}{\Lambda_+} & \text{if $\Effect{t_i} > 0$.}
%%     \end{cases}
%%   \end{gather*}
%%   Recall that we assume that for some $i$, $\Effect{t_i} < 0$.
%%   It follows that $\Lambda_- < 0$.
%%   Additionally, recall that effects of transitions are integers,
%%   therefore so are $\Lambda_-$ and $\Lambda_+$.
%%   It is then easy to see that $\beta_i \in \QZeroOne$ for all $i$.

%%   Let $\phi = \beta_1 t_1 \dots \beta_n t_n$. It follows that
%%   \begin{gather*}
%%     b + \Effect{\phi} = b + \dfrac{-1}{\Lambda_-} \Lambda_- + \dfrac{0.5}{\Lambda_+} \Lambda_+ = b - 0.5 = b'.
%%   \end{gather*}
%%   So $\phi$ has the right effect to obtain $b'$ when starting at $b$.
%%   For ease of notation, we write $a_i = a + \Effect{\FromTo{\rho}{1}{i}}$, $b_i = b + \Effect{\FromTo{\phi}{1}{i}}$, and $c_i = c + \Effect{\FromTo{\sigma}{1}{i}}$.
%%   By \autoref{lemma:follower}, we can assume that $a_i \leq c_i$ for all $i$.

%%   We make a case distinction. First, assume we have some value $i$ such that that either $b_i > c_i$ or $b_i < a_i$. Choose $i$ as the greatest such value. Without loss of generality, let us assume that $b_i < a_i$; the other case follows by symmetry. Then for $j$ such that $i+1 \leq j \leq n$, it holds that
%%   $a_j \leq b_j \leq c_j$, so $b_j \in \guard{\pi_j}$.
%%   Additionally, it holds that $b_{i+1} > a_{i+1}$.
%%   Therefore by \autoref{lemma:follower} there exists $\alpha'$ such that $a_i \steps{\alpha' t_i} b_{i+1}$.
%%   So the run $\rho' = \FromTo{\rho}{1}{i-1} (\alpha' t_i) \FromTo{\phi}{i+1}{n}$ is admissible from $a$ and therefore $a \steps{\rho'} b'$. Since $a \in \Post{\pi^+}{\mathcal{J}}$, it follows that $b' \in \Post{\pi^+}{\mathcal{J}}$.

%%   \newcommand{\newc}{\overline{c}}
%%   \newcommand{\newrun}{\psi}
%%   \newcommand{\finalrun}{\omega}

%%   So it remains to show the case where for all $i$, $a_i \leq b_i \leq c_i$.
%%   We make another case distinction.
%%   If $\Effect{\rho} = \Effect{\sigma} = 0$, then note that $a = a'$, $c = c'$.
%%   Therefore, $a', c' \in \enab{\pi} \cap \Post{\pi^+}{\mathcal{J}}$.
%%   Recall we assume there exists $t_i \in \pi$ such that $\effect{t_i} < 0$.
%%   Let us write $\sigma = \gamma_1 t_1 \dots \gamma_n t_n$.
%%   Then we define
%%   \begin{gather*}
%%     \gamma'_i = \begin{cases}
%%       \dfrac{\gamma_i}{2} & \text{if } \effect{t_i} \geq 0 \\
%%       1                   & \text{if } \effect{t_i} < 0.
%%     \end{cases}
%%   \end{gather*}
%%   Let us define the run $\sigma' = \gamma'_1 t_1 \dots \gamma'_n t_n$.
%%   By definition of $\gamma'$, holds that $\effect{\sigma'} < \effect{\sigma} = 0$.
%%   Let us define $(\newc_i)_j = c + \effect{\sigma'^{j-1}} +
%%     \effect{\FromTo{\sigma'}{1}{i}}$.
%%   Since $\effect{\sigma'} < 0$, it holds that $(\newc_i)_{j+1} < (\newc_i)_{j}$ for all $j$.
%%   Therefore, there must be some smallest $j$ such that there is some
%%   smallest $i$ such that $(\newc_i)_{j} < a_i$.
%%   By \autoref{lemma:follower}, it then holds that there exists some run
%%   $\finalrun$ such that $c \steps{\finalrun} a_i \steps{\FromTo{\rho}{i+1}{n}} a'$.
%%   Therefore $c \steps{\pi^+} a'$. By definition, also $c \steps{\pi^+} c'$. We can write $b' = (1-\Lambda) a' +  \Lambda c'$, since $a' < b' < c'$. By \autoref{lemma:convex}, it follows that $(1-\Lambda) c + \Lambda c \steps{\pi^+} b'$.
%%   Since $(1 - \Lambda) c + \Lambda c = c$, it holds that $c \steps{\pi^+} b'$, so $b' \in \Post{\pi^+}{\mathcal{J}}$.

%%   \michael{\autoref{lemma:convex} deals with paths, not languages; so
%%     is its usage safe here?}

%%   \philip{no, it's a mistake, it can't directly be invoked.}


%%   Let us reason about the case where $\Effect{\sigma} < 0$ or $\Effect{\rho} < 0$.
%%   The case where $\Effect{\sigma} > 0$ or $\Effect{\rho} > 0$ is symmetric.
%%   Let us denote as $\newrun$ the run among $\sigma$
%%   and $\rho$ with the smaller effect.
%%   Let us denote $\newc_j = c + \Effect{\newrun^j}$.
%%   Further, let us denote
%%   $(\newc_j)_i = \newc_{j} + \Effect{\FromTo{\newrun}{1}{i}}$.
%%   It is clear that for all $j, j', i$ such that $j < j'$ it is the case
%%   that $(\newc_j)_i < (\newc_j')_i$, since $\Effect{\newrun} < 0$.

%%   Let $j$ be the smallest value such that $(\newc_j)_i < b_i$.
%%   Then it must hold that $\newrun^j$ is admissible from $c$,
%%   since for all $(\newc_j')_i'$ with $j' < j$, it holds that
%%   $a_i' \leq b_i' \leq (\newc_j')_i' \leq c_i'$. Since $a_i', c_i' \in \guard{\pi_i'}$, therefore $(\newc_j')_i' \in \guard{\pi_i'}$.
%%   Further, note that $(\newc_j)_{i-1} \geq b_{i-1}$.
%%   \philip{This is technically not correct, since $i$ might be $0$, and it gets a bit weird. Something to fix later}
%%   By \autoref{lemma:follower}, it holds that there is some $\beta'$ such that
%%   $(\newc_j)_{i-1} \steps{\beta' t_{i-1}} b_i$.

%%   \michael{I wonder why there are several cases. It'd help me if we
%%     could discuss what is wrong with this approach: We start from $c$
%%     and go to $b'$ by using the negative transition. If it's
%%     admissible, then we are done. Otherwise, we must cross the run
%%     from $a$. So $c \steps{\pi^+} a'$ by
%%     \autoref{lemma:follower}. Since $c \steps{\pi^+} c'$ as well, we
%%     have $c \steps{\pi^+} b'$ by convexity (assuming we can invoke
%%     convexity, which I'm not sure we can). Since this approach is a
%%     part of the current proof, I guess there is a problem with just
%%     doing this?}

%%   \philip{
%%     I agree, what you propose seems like it should work.
%%     I don't think we can invoke convexity directly, however.
%%     We can discuss in the meeting later today
%%   }

%%   \philip{Addendum: I realize why there are several cases. Since convexity
%%   is not applicable, we instead use this argument that we go from "almost b'" to b', which introduces the cases: Either the run from almost b' to b' is admissible or not. The case distinction about $\effect{\rho}$ is needed
%%   for this part: "go to $b'$ by using the negative transition".
%%   It feels like one can do away with this, but there are subtleties since
%%   for example, $\rho$ may already scale the negative transition maximally,
%%   but we need to be sure that the run we get is admissible until it crosses the run from $a$, so always smaller than $\rho$.}

%%   Let us define $\finalrun = \newrun^j \FromTo{\newrun}{1}{i-1} (\beta' t_i) \FromTo{\phi}{i+1}{n}$.
%%   It holds that $\finalrun$ is admissible from $c$. This follows from the fact that $\newrun^j \FromTo{\newrun}{1}{(i-1)}$ is admissible from $c$,
%%   and by assumption $\phi$ is admissible from $b$, and in particular $\FromTo{\phi}{i+1}{n}$ is admissible from $b_i$. Finally, let us note that by definition, $b_i + \Effect{\FromTo{\phi}{(i+1)}{n}} = b'$, so $c \steps{\finalrun} b'$, therefore $b' \in \Post{\pi^+}{\mathcal{J}}$.
%% \end{proof}

\newcommand{\tstar}{\theta^*}
\newcommand{\tplus}{\theta^+}

\newcommand{\J}{\mathcal{J}}

Let us fix a linear guarded COCA $\W = (Q, T, \tau)$
such that $\SPaths{\W} = 
L(\pi_0 \tstar_1 \pi_1 \tstar_2 \dots \pi_{k-1} \tstar_k \pi_k)$. 
Note that by definition, such a decomposition exists for any linear COCA.

\michael{@(F|Ph)ilip: See appendix regarding these lemmas.}

Let
\begin{gather*}\Lambda_i = 
  L(\pi_0 \tstar_1 \pi_1 \tstar_2 \dots \tstar_{i-1} \pi_{i-1} 
  \tplus_i 
  \pi_{i} \pi_{i+1} \dots \pi_k).
\end{gather*} Further, let $\mathcal{J}$ be a finite union of intervals.
Additionally, let us define for the sake of notation
$\hi{\Lambda_i}(x) = \sup(\Post{\Lambda_i}{x}),
  \lo{\Lambda_i}(x) = \inf(\Post{\Lambda_i}{x})$.

\begin{lemma}
  It is the case that $\enab{\Lambda_i}$ is a union
  of at most $i$ intervals for all $i$.
\end{lemma}
\begin{proof}
  We can write $\Lambda_i$ as the union of $i$ sets $\Lambda_{i, 1}$ through $\Lambda_{i,i}$ where
  \begin{gather*}
    \Lambda_{i,j} = 
    L(\pi_0 \dots \pi_{j-1} 
    \tplus_j 
    \pi_{j} \tstar_{j+1} \pi_{j+1} \dots \tstar_{i-1} \pi_{i-1} 
    \tplus_i
    \pi_i \dots \pi_k).
  \end{gather*}
  
  \philip{\dots this proof has to be finished still, and probably relies on something that currently comes after it, i.e. \autoref{lemma:cycle-acceleration}}

\end{proof}

\begin{lemma}
  It is the case that $\Post{\Lambda_i}{\J}$ is an interval for all $i$.
\end{lemma}
\begin{proof}
  Let us first note that $\Lambda_i = X Y Z$ with 
  $X = L(\pi_0 \tstar_1 \pi_1 \tstar_2 \dots \tstar_{i-1} \pi_{i-1})$, 
  $Y = L(\tplus_i)$, 
  $Z = L(\FromTo{\pi}{i}{k})$.
  By definition, $\Post{\Lambda_i}{\J} = 
  (\Post{Z}{} \circ \Post{Y}{} \circ \Post{X}{})(\J)$.

  Let us first show that $\Post{X}{\J} = \mathcal{X}$, where $\J_0$ is a finite union of intervals.
  Note that we can write $X$ as a union of exponentially many sets:
  \begin{gather*}
    X = \bigcup_{j \leq 2^{i-1}} X_j = \bigcup_{l_1 \dots l_{i-1} \in \{0, +\}} \pi_0 \theta^{l_1} \pi_1 \dots \pi_{i-1} \theta^{l_{i-1}} \pi_{}.
  \end{gather*}
  By \autoref{lemma:postplus_interval} and \autoref{lemma:post-intervals}, 
  it holds that $\Post{X_j}{\J}$ is an interval. 
  Therefore, $X' = \Post{X}{\J}$ is a finite union of intervals.
  Further, note that $Y' = \Post{Y}{X'} = \Post{\tplus_i}{X'}$.
  Hence, $Y'$ is an interval by \autoref{lemma:postplus_interval}.
  Lastly it follows that $\Post{\Lambda_i}{\J} = \Post{Z}{Y'}$ is an interval by \autoref{lemma:post-intervals}.
\end{proof}

\michael{See appendix for a reformulation of this lemma.}

\begin{lemma}\label{lemma:path-hilo}
  Let $\pi$ be a path of $\W$.
  There exist constants $x, x', y, y' \in \Q$ such for all $a \in \enab{\pi}$,
  it is the case that \begin{itemize}
    \item $\hi{\pi}(x) = \min(x + x, x')$,
    \item $\lo{\pi}(x) = \max(x + y, y')$.
  \end{itemize}
\end{lemma}
\begin{proof}
  We prove the case where $\pi$ is a single transition $t$.
  The general case follows by induction.

  Let us write $\delta_t = \Effect{t}$, $\tau_t = \guard{\Out{t}}$.
  It holds that by definition $\Post{t}{a} = \{b \mid a \steps{t} b\} = 
  \{b \in \tau_t \mid b = a + \alpha t \wedge \alpha \in \ZeroOne\}$.

  If $\effect{t} = 0$, then $\hi{t}(a) = a = \min(a + 0, \sup(\enab{t}))$ and 
  $\lo{t}(a) = a = \max(a + 0, \inf(\enab{t}))$, 
  since we assume $a \in \enab{t}$.
  If $\effect{t} > 0$, then $\hi{t}(a) = \min(a + \delta_t, \sup(\tau_t))$ and
  $\lo{t}(a) = \max(a, \inf(\tau_t)$. The case $\effect{t} < 0$ is symmetric.

  \philip{maybe we need to show the induction step here, maybe not}
\end{proof}

In the following, we fix some cycle $\theta = t_1 \dots t_n$ of $\W$.
Let us define $q_0 = \In{t_1}$, $q_i = \Out{t_i}$ for $1 \leq i \leq n$.

\michael{What is $\J$ here? This symbol has been used as a finite
  union of intervals so far. But if it is here , then the statement is
  misleading as $\mathrm{Post}_{\pi}(\J)$ is not necessarily an
  interval. Also, $\varepsilon$ has been used as the empty path.}

\philip{it indeed is supposed to be a finite union of intervals.
Note that even non-interval sets have a supremum, so I don't think there is a contradiction}

\begin{lemma}\label{lemma:sup-enab}
  Let $\pi$ be a path. 
  \begin{enumerate}[label=\Roman*)]
    \item \label{item:sup}
      It holds that $\hi{\pi}(\mathcal{J}) = \hi{\pi}(\sup(\mathcal{J} \cap \enab{\pi}))$.
    \item \label{item:inf}
    It holds that $\lo{\pi}(\mathcal{J}) = \lo{\pi}(\inf(\mathcal{J} \cap \enab{\pi}))$.
  \end{enumerate}
\end{lemma}
\philip{One use of the good \autoref{lemma:follower} where everything is a run, one use of the "not-so-bad" single-transition version}
\begin{proof}
  \newcommand{\hc}{h}
  \newcommand{\hcepsilon}{h_{\varepsilon}}
  We prove \ref{item:sup}; then \ref{item:inf} follows by symmetry.

  We assume that $\pi = t_1 \dots t_n$.
  Let us denote $\hc = \sup(\mathcal{J} \cap \enab{\pi})$ and $\hc' = \hi{\pi}(\hc)$.
  We first prove $\hi{\pi}(\mathcal{J}) \leq \hc'$.
  By definition of $\hi{\pi}$, there must be some $k \in \ZeroOne$ such that 
  $\hc \steps{\pi} \hc' - \varepsilon$ for all $\varepsilon < k$.
  Let us fix an arbitrary such $\varepsilon$, and let us write $\hcepsilon = \hc' - \varepsilon$.
  Assume for the sake of contradiction there exists $a \in \mathcal{J}$ such that $\hi{\pi}(a) > \hc'$.
  Let us denote $a' = \hi{\pi}(a)$.
  It must hold that $a \in enab{\pi}$, hence $a < \hc$. Since $a \steps{\pi} a'$, 
  $\hc \steps{\pi} \hcepsilon$ and $a < \hc$, $a' > hc' > \hcepsilon$,
  by \autoref{lemma:follower} it follows that $\hc \steps{\pi} a'$. This is a contradiction, since $a' > \hc' = \hi{\pi}(\hc)$.
  So $\hi{\pi}(\mathcal{J}) \leq \hc'$.

  It remains to show that $\hi{\pi}(\mathcal{J}) \geq \hc'$.
  It suffices to show that there exists $k'$ such that $\hc' - \varepsilon' \in \Post{\pi}{\mathcal{J}}$ for all $\varepsilon' < k'$,
  By definition of $\sup$, there exists $k$ such that $\hc - \varepsilon \in \mathcal{J} \cap \enab{\pi}$ for $\varepsilon < k$.
  Additionally, there exists $l'$ such that $\hc' - \delta' \in \Post{\pi}{\hc}$ for $\delta' < l'$.
  Let us define $k' = \min(k, l')$. For all $\varepsilon' < k'$, it holds that $\hc - \dfrac{\varepsilon'}{2} \in \mathcal{J} \cap \enab{\pi}$,
  since $\dfrac{\varepsilon'}{2} < k$.  By a similar argument, it holds that $\hc' - \dfrac{\varepsilon'}{2} \in \Post{\pi}{\hc}$.
  Hence, there exists some run $\rho$ with $\upath{\rho} = \pi$ such that $\hc \steps{\rho} \hc' - \dfrac{\varepsilon'}{2}$.
  Let us apply $\rho$ to $\hc - \dfrac{\varepsilon'}{2}$.
  It holds that 
  \begin{gather*}
    \hc - \dfrac{\varepsilon'}{2} + \effect{pi} = \\
    \hc - \dfrac{\varepsilon'}{2} + (\hc' - \dfrac{\varepsilon'}{2} - \hc) = \\
    \hc' - \dfrac{\varepsilon' + \varepsilon'}{2} = \\
    \hc' - \varepsilon.
  \end{gather*}
  If $\rho$ is admissible from $\hc - \dfrac{\varepsilon'}{2}$, we are done.
  Otherwise, note that $\hc - \dfrac{\varepsilon'}{2} \in \enab{\pi}$, so there must exist some run $\sigma$ with $\upath{\sigma} = \pi$
  such that $\hc - \dfrac{\varepsilon'}{2} \steps{\sigma} b'$.
  Let us denote $h_i = \hc - \dfrac{\varepsilon'}{2} + \effect{\FromTo{\rho}{1}{i}}$, $b_i = \hc - \dfrac{\varepsilon'}{2} +\effect{\FromTo{\Sigma}{1}{i}}$. If $b' \geq \hc'$, we are done, since then clearly $\hi{\pi}(\mathcal{J}) \geq \hc'$.
  So assume $b' < \hc'$.
  If $b_i \geq h_i$ for all $i$, then $\rho$ is admissible from $\hc - \dfrac{\varepsilon'}{2}$, since $\rho$ is admissible from $\hc > \hc - \dfrac{\varepsilon'}{2}$. So assume $b_i < h_i$ for some $i$. Let $j$ be the largest index such that $b_i < h_i$.
  In particular, it must hold that $b_{j+1} \geq h_{j+1}$. Then by \autoref{lemma:follower}, it holds that
  there exists some $\alpha t_j$ such that $h_i + \alpha t_j = b_{j+1}$. Then note that
  \[ \hc - \dfrac{\varepsilon'}{2} \steps{\FromTo{\sigma}{1}{j-1}} h_j \steps{\alpha t_j} b_{j+1} \steps{\FromTo{\rho}{j+1}{n}} \hc' - \varepsilon'.\]
  So  $\hc' - \varepsilon' \in \Post{\pi}{\mathcal{J}}$.
\end{proof}

Let us denote as $\bot = \max_{0 \leq i \leq n}(\inf(\guard{q_i}))$, $\top = \min_{0 \leq i \leq n}(\sup(\guard{q_i}))$.
Intuitively, $\bot$ is the highest bottom-guard, while $\top$ is the lowest top-guard.
Then we define the sets $L = \{i \mid \inf(\guard{q_i}) = \bot\}$ and $H = \{i \mid \sup(\guard{q_i}) = \top\}$.

\begin{lemma}\label{lemma:cycle-acceleration}
  Let $a \in \enab{\theta}$.
  \begin{enumerate}[label=\Roman*)]
    \item \label{item:hi}
          If $\effect{t} > 0$ for some $t \in \theta$,
          then it holds that $\hi{\theta^+}(a) = 
          \hi{\FromTo{\theta}{(i+1)}{n}}(\top)$
          for all $i \in H$.
    \item\label{item:lo}
          If $\effect{t} < 0$ for some $t \in \theta$, 
          then it holds that $\lo{\theta^+}(a) = 
          \lo{\FromTo{\theta}{(i+1)}{n}}(\bot)$ 
          for all $i \in L$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  Let us prove \ref{item:hi}. Then \ref{item:lo} follows by symmetry.
  
  Let us write $\theta' = \FromTo{\theta}{1}{i}$, $\theta'' =  \FromTo{\theta}{i+1}{n}$.
  Let us write $\phi = L(\theta^* \theta')$.
  It holds that $\Post{\theta^+}{a} = \Post{\phi \theta''}{a} = \Post{\theta''}{\Post{\phi}{a}}$.
  Then by \autoref{lemma:sup-enab}, it holds that $\hi{\theta''}(\Post{\phi}{a}) = \hi{\theta''}(\sup(\Post{\phi}{a} \cap \enab{\theta''}))$.
  So it suffices to show that $\top = \sup(\Post{\phi}{a} \cap \enab{\theta''})$.
  Note that $a \in \enab{\theta}$, by assumption. So there exists some run $\rho = \alpha_1 t_1 \dots \alpha_n t_n$ such
  that $a \steps{\rho} a'$ for some $a'$. Let us denote $a_j = a + \effect{\FromTo{\rho}{1}{j}}$.

  Let us first show that $\top \leq \sup(\Post{\phi}{a} \cap \enab{\theta''})$.
  Note that $\Post{\phi}{a}$ and $\enab{\theta''})$ are intervals, by definition of $\enab{\theta''}$
  and \autoref{lemma:postplus_interval}. Then we need to show that $\top \in \cl{\Post{\phi}{a} \cap \enab{\theta''})}$.

  If $a_i = \top$, then clearly we are done. So assume $a_i < \top$.
  Hence, we show that for any $k > 0$, there exists some $0 \leq \kappa < k$ such that $\top - \kappa \in \Post{\phi}{a} \cap \enab{\theta''}$.
  Let us choose $\varepsilon = \min(\top - a_i, k, 0.5)$. 
  Note that $\varepsilon > 0$, since $\top > a_i$.
  We define $\delta_+ = \sum_{1 \leq j \leq n}{max(0, \effect{t_i}}$ and $\delta_- = \sum_{1 \leq j \leq n}{min(0, \effect{t_i}}$.
  Then for $1 \leq j \leq n$, we let \begin{gather*}
    \gamma_j = \begin{cases}
      \dfrac{\varepsilon}{8 \delta_+} & \text{if } \effect{t_j} \geq 0 \\
      -\dfrac{\varepsilon}{8 \delta_-} & \text{if } \effect{t_j} < 0.
    \end{cases}
  \end{gather*}

  Recall that we assume that $\effect{t} > 0$ for some $t \in \theta$.
  Then $\delta_+ \geq 1$ (since effects of transitions are integers), and $\delta_- \leq -1$ if there exists some $t \in \theta$ with $\effect{t} < 0$.
  Also, note that $\varepsilon < 1$. Then it is clear that $\gamma_j \in \ZeroOne$ for all $j$.
  Let us define the run $\sigma = \gamma_1 t_1 \dots \gamma_n t_n$ and $b = \top - \dfrac{\varepsilon}{2}$.
  For $0 \leq j \leq n$, we write $b_j = b + \effect{\FromTo{\sigma}{1}{j}}$ and 
  $b_{n+j} = b + \effect{\sigma} + \effect{\FromTo{\sigma}{1}{j}}$.
  
  Let us show that for all $j \leq n$, $\top - \varepsilon \leq b_j \leq \top$ and $\top - \varepsilon \leq b_{n+j} \leq \top$.
  It holds that $b_j \leq b + \dfrac{\varepsilon}{8 \delta_+} \delta_+ 
  < b + \dfrac{\varepsilon}{2} = \top$ and
  $b_{n+j} \leq 
  b + \dfrac{\varepsilon}{8 \delta_+} \delta_+ + \dfrac{\varepsilon}{8 \delta_+} \delta_+ < b + \dfrac{\varepsilon}{2} = \top$.
  Additionally, we have that $b_j = \geq b - \dfrac{\varepsilon}{8 \delta_-} \delta_- \geq b - \dfrac{\varepsilon}{2} = \top - \varepsilon$
  and $b_{n+j} \geq b - \dfrac{\varepsilon}{8 \delta_-} \delta_- \dfrac{\varepsilon}{8 \delta_-} \delta_- \geq b - \dfrac{\varepsilon}{2} = \top - \varepsilon$.

  There are three cases:
  The first is when $a_j > b_j$ for all $0 \leq j \leq n$. Then note that, in particular, $a_i > b_i > \top - \varepsilon$.
  Then we are done since $a_i \in \Post{\phi}{a}$ and $a_i \in \enab{\theta''}$, and $a_i > \top - \varepsilon \geq \top - \kappa$.

  The second case is when $a_j < b_j$ for all $0 \leq j \leq n$.
  In this case, we show that $b_{n+i} \in \Post{\phi}{a} \cap \enab{\theta''}$.
  Since there is some $t \in \theta$ with $\effect{t} > 0$, let us rescale $\rho$ into a run with a larger effect that is guaranteed to be positive.
  Formally speaking, let us take the run $\rho' = \alpha'_1 t_1 \dots \alpha'_n t_n$, where
  \begin{gather*}
    \alpha'_i = \begin{cases}
      1 & \text{if } \effect{t_i} \geq 0 \\
      \min(\alpha_i, -\dfrac{1}{2 \delta^-}) & \text{if } \effect{t_i} < 0
    \end{cases}
  \end{gather*}
  
  \newcommand{\newa}{\overline{a}}
  
  It holds that $\effect{\rho'} \geq \delta_+ - \dfrac{1}{2 \delta^-} \delta^- = \delta_+ - \dfrac{1}{2} \geq \dfrac{1}{2}$, since
  $\delta_+ \geq 1$ by the assumption that there exists a transition with positive effect on $\theta$.
  Additionally, it is easy to see that $\effect{\rho'} \geq \effect{\rho}$.
  Let us define $(\newa_j)_l = a + \effect{\rho'^j} + \effect{\FromTo{\rho'}{1}{l}}$.
  Clearly, $(\newa_j)_0 < (\newa_{j+1})_0$, since $\effect{\rho'} > 0$.
  So there must exist some $j, l$ such that $(\newa_j)_l > b_l$. In particular, it must then hold that $(\newa_j)_{l-1} \leq b_{l-1}$
  \philip{there is a minor problem when $l=0$, probably needs an additional case distinction}
  Let us choose the minimal such $j$ and the minimal such $l$ for the chosen $j$.
  Note that for all $0 \leq j \leq n$, $b_j < \top$, hence $b_j \in \topguard{\pi_j}$.
  In words, all configurations we obtain 
  by run $\sigma$ when starting on $b$ satisfy the upper bound of the respective state.
  Hence $\rho'^j \FromTo{\rho'}{1}{l}$ is admissible from $a$, since for all $j', l'$,
  $a_l' \leq (\newa_j')_l' \leq b_l'$.
  Additionally, by \autoref{lemma:follower$}, it holds that there exists some $\beta'$ such that 
  $(\newa_j)_{l-1} \steps{\beta' t_{l-1}} b_{l}$. Lastly, note that $\FromTo{\sigma}{l+1}{n} \sigma$ is admissible from $b_l$
  by the fact that $a_l' \leq b_l' \leq b_{n+l'}$.
  Then $a \steps{\rho^j \FromTo{\rho}{1}{l-1}}(\newa_j)_{l-1} \steps{\beta' t_{l-1}} b_{l} \steps{\FromTo{\sigma}{l+1}{n}\FromTo{\sigma}{1}{i}} 
  b_{n+i} \steps{\FromTo{\sigma}{i+1}{n}} b_{2n}$.
  Lastly, note that $\upath{\rho^j \FromTo{\rho}{1}{l-1} \beta' t_{l-1} \FromTo{\sigma}{l+1}{n}\FromTo{\sigma}{1}{i}} \in \phi$,
  and $\upath{\FromTo{\sigma}{i+1}{n}} = \theta''$.
  Therefore, $b_{n+i} \in \Post{\phi}{a} \cap \enab{\theta''}$, and we are done since $b_{n+1} \geq \top - \varepsilon \geq \top - \kappa$.
  
  The last case is when there is some $j$ such that either $a_j \leq b_j$ and $a_{j+1} > b_{j+1}$ or
  $a_j \geq b_j$ and $a_{j+1} < b_{j+1}$. 
  
  Let us first handle the case where $a_j \leq b_j$ and $a_{j+1} > b_{j+1}$ holds.
  Note that for some $j'$, if it holds that $a_{j'} \leq b_{j'}$, then also $b_{j'} \in \guard{\pi_{j'}}$:
  This follows from the fact that $b_{j'} < \top$, hence $b_{j'} \in \topguard{\pi_{j'}}$, and the fact that $a_{j'} \in \guard{\pi_{j'}}$,
  hence in particular $a_{j'} \in \botguard{\pi_{j'}}$.
  Note that by choice of $\varepsilon$, $a_i \leq b_i$. If $a_i = b_i$, we are done, so let us assume $a_i < b_i$.
  Then let us 


  

  \philip{the idea is: follow $\rho$ or $\sigma$, whichever is larger. then we must at least reach $b_i$, therefore done}






\end{proof}

